Search results diversification in competitive search

In Web retrieval, there are many cases of competition between authors of Web documents: their incentive is to have their documents highly ranked for queries of interest. As such, the Web is a prominent example of a competitive search setting. Past work on competitive search focused on ranking functions based solely on relevance estimation. We study ranking functions that integrate a results-diversification aspect. We show that the competitive search setting with diversity-based ranking has an equilibrium. Furthermore, we theoretically and empirically show that the phenomenon of authors mimicking content in documents highly ranked in the past, which was demonstrated in previous work, is mitigated when search results diversification is applied.

==> Tables/consWinnersEmbeddings.tex <==
\begin{tabular}{l|cccc}
&   {E5 (\baseShort, \divShort)} & {SBERT (\baseShort, \divShort)} & {TF.IDF (\baseShort, \divShort)} & {Jaccard (\baseShort, \divShort)} \\ \toprule
Mean similarity      & $0.97$, $0.95^{*}$ & $0.93$, $0.87^{*}$ & $0.89$, $0.76^{*}$ & $0.66$, $0.55^{*}$ \\
\bottomrule
\end{tabular}

==> Tables/consWinnersFeatures.tex <==
\begin{tabular}{l|ccc}
Query-dependent & {TF (\baseShort, \divShort)} & {BM25 (\baseShort, \divShort)} & {LM.DIR (\baseShort, \divShort)} \\ \toprule
 Absolute difference & $2.17$, $3.24$ & $0.3$, $1$ & $0.37$, $0.95$ \\ \midrule
 Query independent & {Length (\baseShort, \divShort)} & {StopwordRatio (\baseShort, \divShort)} & {Entropy (\baseShort, \divShort)} \\ \toprule
Absolute difference & $8.03$, $9.39$ & $0.02$, $0.05$ &$0.07$, $0.12$ \\ \bottomrule
\end{tabular}



==> Tables/genStats.tex <==
\begin{tabular}{|l|c|c|c|c|}
\hline
\textbf{Feature /\ Representation} & \textbf{E5 (B, D)} & \textbf{SBERT (B, D)} & \textbf{TF-IDF (B, D)} & \textbf{JACCARD (B, D)} \\ 
\hline
Average group similarity      & $0.94$, $0.9$ & $0.85$, $0.77$ & $0.74$, $0.61$ & $0.44$, $0.35$ \\
\hline
Diameter group similarity& $0.91$, $0.85$ & $0.8$, $0.67$ & $0.65$, $0.46$ & $0.32$, $0.22$ \\
\hline
Between-average group similarity& $0.05$, $0.07$ & $0.1$, $0.12$ & $0.18$, $0.17$ & $0.22$, $0.17$ \\
\hline
Within-average group similarity& $0.02$, $0.04$ & $0.05$, $0.09$ & $0.08$, $0.13$ & $0.13$, $0.15$ \\
\hline
\end{tabular}


==> Tables/tmpTransMatrix.tex <==

\omt{
\[
\begin{array}{c|cccc}
    Position@ t \backslash Position@ {(t+1)} & 1 & 2 & 3 & 4 \\
    \hline
    1 & \textbf{0.68} & \textbf{0.26} & 0.03 & 0.03 \\
    2 & 0.07 & 0.46 & 0.42 & 0.06 \\
    3 & 0.17 & 0.20 & 0.34 & 0.29 \\
    4 & 0.09 & 0.09 & 0.20 & 0.62 \\
\end{array}
\]
\captionof{table}{The baseline transition matrix shows the probabilities of transitioning from each position at round \( t \) to each position at round \( t+1 \) in competition \textbf{B}.}
\label{transition_b}

\[
\begin{array}{c|cccc}
    Position@ t \backslash Position@ {(t+1)} & 1 & 2 & 3 & 4 \\
    \hline
    1 & \textbf{0.63} & 0.11 & \textbf{0.23} & 0.02 \\
    2 & 0.11 & 0.58 & 0.13 & 0.18 \\
    3 & 0.17 & 0.12 & 0.40 & 0.31 \\
    4 & 0.09 & 0.19 & 0.23 & 0.49 \\
\end{array}
\]
%\captionof{table}{The diversity transition matrix shows the probabilities of transitioning from each position at round \( t \) to each position at round \( t+1 \) in competition \textbf{D}.}
\label{transition_d}
}


==> Tables/transMatrix,v2.tex <==
\begin{tabular}{c|cccc}
  \multicolumn{5}{c}{\textbf{Baseline}} \\ \hline
  % Header Row
  Position@t$\backslash$ Position@(t+1) & 1 & 2 & 3 & 4 \\ \hline
  1 & $0.68$ & $0.26$ & $0.03$ & $0.03$ \\
  2 & $0.07$ & $0.46$ & $0.42$ & $0.06$ \\
  3 & $0.17$ & $0.20$ & $0.34$ & $0.29$ \\
  4 & $0.09$ & $0.09$ & $0.20$ & $0.62$ \\ \hline
  \multicolumn{5}{c}{\textbf{Diversity}} \\ \hline
  1 & $0.68$ & $0.26$ & $0.03$ & $0.03$ \\
  2 & $0.07$ & $0.46$ & $0.42$ & $0.06$ \\
  3 & $0.17$ & $0.20$ & $0.34$ & $0.29$ \\
  4 & $0.09$ & $0.09$ & $0.20$ & $0.62$ \\
\end{tabular}


==> ack.tex <==

\smallskip
\myparagraph{Acknowledgments} We thank the reviewers for their comments.
The work by Moshe Tennenholtz was supported by funding from the
European Research Council (ERC) under the European Union's Horizon
2020 research and innovation programme (grant agreement 740435).


==> figs/strategies/B/query_dependent.tex <==
\begin{figure}
\centering
\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{../figures//lv_local/home/tommymordo/PycharmProjects/pythonProject/Analyzer_diversity2/experiments/graphs/query_dependent/okapi_improvers}
  \caption{Okapi}
  \label{fig:okapi}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{../figures//lv_local/home/tommymordo/PycharmProjects/pythonProject/Analyzer_diversity2/experiments/graphs/query_dependent/languagemodel_improvers}
  \caption{LanguageModel}
  \label{fig:languagemodel}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{../figures//lv_local/home/tommymordo/PycharmProjects/pythonProject/Analyzer_diversity2/experiments/graphs/query_dependent/termfrequency_improvers}
  \caption{TermFrequency}
  \label{fig:termfrequency}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{../figures//lv_local/home/tommymordo/PycharmProjects/pythonProject/Analyzer_diversity2/experiments/graphs/query_dependent/normalizedtermfrequency_improvers}
  \caption{NormalizedTermFrequency}
  \label{fig:normalizedtermfrequency}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{../figures//lv_local/home/tommymordo/PycharmProjects/pythonProject/Analyzer_diversity2/experiments/graphs/query_dependent/bert_improvers}
  \caption{BERT}
  \label{fig:bert}
\end{subfigure}%
\medskip

\caption{Query Dependent Features: Comparison of averaged query-dependent feature values for documents that shifted from losing to winning...}
\label{fig:query-dependent}
\end{figure}

==> figs/strategies/B/query_independent.tex <==
\begin{figure}
\centering
\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{../figures//lv_local/home/tommymordo/PycharmProjects/pythonProject/Analyzer_diversity2/experiments/graphs/query_independent/entropy_improvers}
  \caption{Entropy}
  \label{fig:entropy}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{../figures//lv_local/home/tommymordo/PycharmProjects/pythonProject/Analyzer_diversity2/experiments/graphs/query_independent/stopwordsratio_improvers}
  \caption{StopWordsRatio}
  \label{fig:stopwordsratio}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{../figures//lv_local/home/tommymordo/PycharmProjects/pythonProject/Analyzer_diversity2/experiments/graphs/query_independent/stopwordscover_improvers}
  \caption{StopWordsCover}
  \label{fig:stopwordscover}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{../figures//lv_local/home/tommymordo/PycharmProjects/pythonProject/Analyzer_diversity2/experiments/graphs/query_independent/documentlength_improvers}
  \caption{DocumentLength}
  \label{fig:documentlength}
\end{subfigure}%
\medskip

\caption{Query Independent Features: Comparison of averaged query-independent feature values for documents that shifted from losing to winning...}
\label{fig:query-independent}
\end{figure}

==> figs/strategies/D/query_dependent.tex <==
\begin{figure}
\centering
\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{../figures//lv_local/home/tommymordo/PycharmProjects/pythonProject/Analyzer_diversity2/experiments/graphs/query_dependent/okapi_improvers}
  \caption{Okapi}
  \label{fig:okapi}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{../figures//lv_local/home/tommymordo/PycharmProjects/pythonProject/Analyzer_diversity2/experiments/graphs/query_dependent/languagemodel_improvers}
  \caption{LanguageModel}
  \label{fig:languagemodel}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{../figures//lv_local/home/tommymordo/PycharmProjects/pythonProject/Analyzer_diversity2/experiments/graphs/query_dependent/termfrequency_improvers}
  \caption{TermFrequency}
  \label{fig:termfrequency}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{../figures//lv_local/home/tommymordo/PycharmProjects/pythonProject/Analyzer_diversity2/experiments/graphs/query_dependent/normalizedtermfrequency_improvers}
  \caption{NormalizedTermFrequency}
  \label{fig:normalizedtermfrequency}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{../figures//lv_local/home/tommymordo/PycharmProjects/pythonProject/Analyzer_diversity2/experiments/graphs/query_dependent/bert_improvers}
  \caption{BERT}
  \label{fig:bert}
\end{subfigure}%
\medskip

\caption{Query Dependent Features: Comparison of averaged query-dependent feature values for documents that shifted from losing to winning...}
\label{fig:query-dependent}
\end{figure}

==> figs/strategies/D/query_independent.tex <==
\begin{figure}
\centering
\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{../figures//lv_local/home/tommymordo/PycharmProjects/pythonProject/Analyzer_diversity2/experiments/graphs/query_independent/entropy_improvers}
  \caption{Entropy}
  \label{fig:entropy}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{../figures//lv_local/home/tommymordo/PycharmProjects/pythonProject/Analyzer_diversity2/experiments/graphs/query_independent/stopwordsratio_improvers}
  \caption{StopWordsRatio}
  \label{fig:stopwordsratio}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{../figures//lv_local/home/tommymordo/PycharmProjects/pythonProject/Analyzer_diversity2/experiments/graphs/query_independent/stopwordscover_improvers}
  \caption{StopWordsCover}
  \label{fig:stopwordscover}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{../figures//lv_local/home/tommymordo/PycharmProjects/pythonProject/Analyzer_diversity2/experiments/graphs/query_independent/documentlength_improvers}
  \caption{DocumentLength}
  \label{fig:documentlength}
\end{subfigure}%
\medskip

\caption{Query Independent Features: Comparison of averaged query-independent feature values for documents that shifted from losing to winning...}
\label{fig:query-independent}
\end{figure}

==> preliminaries.tex <==
%\section{Background}
\subsection{Game Theory}
\label{sec:gt}
We now briefly review some basic concepts in game theory. 
\begin{definition}
  An n-players game is a tuple $G=(\{S_i\}_{i\in N}, \{U_i\}_{i\in N})$. $S_i$ is the set of strategies of player $i$.
  %\subseteq
  %\mathbb{R_{+}}$
  %  is player $i$'s set of possible strategies\footnote{$\mathbb{R_{+}}$ is the set of non-negative real numbers.}.
  $S=S_1 \times S_2 \times ... \times S_n$ is the set of \textbf{strategy profiles} in the game. $U_i:S\rightarrow \mathbb{R_{+}}$ is the \textbf{utility function} of player $i$.\footnote{$\mathbb{R_{+}}$ is the set of non-negative real numbers.}
\end{definition}

Each player in a game aims to maximize her utility. Note that the utility
depends not only on her strategy but also on the strategies of other
players. Consider the following 2-players game:
$S_1=S_2=[0,1]$, $U_1(s_1, s_2) = 1 + s_1^2 + s_2^2, U_2(s_1, s_2) = 2 + s_1^2 + s_2^2$. If the players select $s_1=1$ and $s_2=1$, then their utilities are
$U_1(1,1) = 3$ and  $U_2(1,1) = 4$.

A fundamental characterization of games is their stability or lack
thereof. A {\em stable} strategy profile of a game is a profile where
no player has an incentive to deviate from her strategy. A well known example of a stable profile is Nash equilibrium. Let $S_{-i} = S_1\times...\times S_{i-1} \times S_{i+1} \times ... \times S_n$ denote the strategy profile of all the players except $i$. Then,
%This principle is commonly known as the
%game's solution.
\begin{definition}
  \label{def:nash}
 A strategy profile $s=(s_i, s_{-i})$ where $s_i \in S_{i}, s_{-i} \in S_{-i}$ is a Nash equilibrium  if$~~$ $\forall i \in N$ and $\forall s_i' \in S_i$, $U_i(s_i', s_{-i}) \leq U_i(s_i, s_{-i})$.\footnote{We focus on pure strategies and pure Nash equilibrium. Mixed strategies which are distributions over pure strategies are outside the scope of this paper.}
\end{definition}
Considering the game example from above, it is easy to show that the strategy profile $s_1=1, s_2=1$ is a Nash equilibrium.

%Regarding Our example, The game has a pure Nash equilibrium: the strategy profile $s_1=1, s_2=1$. As a proof, let observe a deviation of player $i=1$ . In the defined game, $0 \leq s_1 \leq 1, 0 \leq s_2 \leq 1$, and assuming player $i=1$ deviates to strategy $s<1$, then he reduces his utility:  $U_1(s, 1) = 1 + s^2 + 1^2 < U_1(1, 1) = 1 + 1^2 + 1^2$. The same proof holds for the second player. Note that in general, a pure Nash equilibrium in the games we have defined, does not necessarily occur.

A {\em dominant strategy} of a player is a strategy that is better than any other strategy regardless of the strategies of other players:
\begin{definition}
$s_i \in S_i$ is a dominant strategy of player $i$ if$~~$ $\forall s_{-i} \in S_{-i}, \forall s'_{i} \in S_i, U_i(s'_{i}, s_{-i}) \leq U_i(s_i, s_{-i})$.
\end{definition}
Note that players' strategies in a Nash equilibrium (Definition \ref{def:nash}) need not
necessarily be dominant strategies. In our example game, $s_1=1$ is a
dominant strategy of the first player, since $U_1(1,s_2) \geq U_1(s_1,
s_2)$~~$ \forall s_1,s_2 \in [0,1]$.

A common measure of the "goodness" of a strategy profile $s$ is {\em
  social welfare}, often defined as the sum of the players' utilities:
\begin{equation}
  \label{eq:social}
   SW(s) = \sum_{i \in  N} U_i(s).
\end{equation}

\endinput

\subsection{Preliminaries for our setup}
We denote a question with length of $k$ tokens as $q \in \textk$, where $\textk$ is a set of all series of tokens with length of $k$ tokens, and $\voc$ is a vocabulary of tokens. ***Oren***: query or question? ***Tommy***: i fixed to question here and everywhere XXX. ***Oren***: if V is a vocabulary of tokens it should be defined as such ***Tommy***: fixed. ***Oren***: k in math mode. ***Tommy***: fixed. For simplicity, we consider strings with a fixed length of k tokens, and in instances where the string is shorter, we pad it with NULL tokens. ***Oren***: if we pad, we should simply define sequences of k tokens. ***Tommy***: fixed.
In a similar manner, we denote as $\adi \in \textk$ the advertisement of the advertiser $i$ with length of $k$ tokens. \\ $\distk$ is a set of all distributions over the set of all series of tokens with length of $k$.

One of the key element of our research is text similarity. Extensive research has been conducted on comparing texts in two main aspects: \textbf{text distance} and \textbf{text representation}. The text distance can be divided into distribution distance or semantic distance, in both cases we expect the distance decrease when the texts are more "similar". Text representation is divided mainly into string-based distance and semantic-based distance \cite{wang_measurement_2020}. ***Oren***: not exactly; there is lexical distance (tf.idf) which doesn't fall into the category of semantics, depends on which community you ask. ***Tommy***: should i omit this paragraph and only mention there are several approaches defining similarity between texts, and jump to the general definition?
In general, we propose the following definition of similarity metric between two series of tokens:

\begin{definition}
A Similarity Metric between two series of $k$ tokens is defined as:
$S: \textk \times \textk \xrightarrow{} \mathbb{R_{+}}$. \end{definition}

***** Moshe: But $V$ was a set of single tokens, so I do get the below... We need to be here very careful about token vs. string, and where random variables come in to play in all definitions, not to be hidden beyond a symbol like $S$ if used for different kinds of inputs *****
*** Tommy: i fix it and concentrate on series of k tokens for the similarities calculations.***


\endinput
In section XX we define similarity metrics operated on Unigram Language Models (LM) used to represent texts. We use the following definition:
\begin{definition}
A \textit{Uni-gram Language Model} (LM) induced by a document $d \in V^{k}$ is defined as $P\in \Delta(V)$, $P(t|d) = \frac{C(t,d)}{\sum_{t\in d}C(t,d)}$. $\forall t \in V: C(t,d)$ is the number of occurrences of the token $t$ in document $d$.
\end{definition}
****Oren****: p was used as a price above; not good to use the same notation for two different things.
****Tommy****: changed to $P$.

% \begin{definition}
% A Similarity Metric between two language models is defined as
% $S: \Delta(V) \times \Delta(V) \xrightarrow{} \mathbb{R_{+}}$.
% \end{definition}
% An important property of the similarity metric is when it achieves its maximum value. We define a \textit{valid similarity metric}, as a similarity metric that achieves its maximum when the two texts are identical. formally:
***Oren***: This property is called Identity of Indiscernibles;
***Oren***: I am not sure this deserves a definition;
***Tommy***: i omit this for now.
% \begin{definition}
% $S$ is a valid Similarity Metric between two texts iff for every $d_a, d_b \in V^{k}$
% $S(d_a, d_b) \leq S(d_a, d_a)$ and $S(d_a, d_b) \leq S(d_b, d_b)$. \end{definition}
% $\{d_i, \beta_i, b_i\}^{n}_{i=1}$ publishers where

%  In LM text representation, the definition is equivalent:
 
% \begin{definition}
% $S$ is a valid Similarity Metric between two language models iff for every $d_a, d_b \in \Delta(V^{k})$
% $S(d_a, d_b) \leq S(d_a, d_a)$ and $S(d_a, d_b) \leq S(d_b, d_b)$. \end{definition}

